Automating Ambiguity: Challenges and Pitfalls of Artificial Intelligence

Machine learning (ML) and artificial intelligence (AI) tools increasingly permeate every possible social, political, and economic sphere; sorting, taxonomizing and predicting complex human behaviour and social phenomena. However, from fallacious and naive groundings regarding complex adaptive systems to datasets underlying models, these systems are beset by problems, challenges, and limitations. They remain opaque and unreliable, and fail to consider societal and structural oppressive systems, disproportionately negatively impacting those at the margins of society while benefiting the most powerful. The various challenges, problems and pitfalls of these systems are a hot topic of research in various areas, such as critical data/algorithm studies, science and technology studies (STS), embodied and enactive cognitive science, complexity science, Afro-feminism, and the broadly construed emerging field of Fairness, Accountability, and Transparency (FAccT). Yet, these fields of enquiry often proceed in silos. This thesis weaves together seemingly disparate fields of enquiry to examine core scientific and ethical challenges, pitfalls, and problems of AI. In this thesis I, a) review the historical and cultural ecology from which AI research emerges, b) examine the shaky scientific grounds of machine prediction of complex behaviour illustrating how predicting complex behaviour with precision is impossible in principle, c) audit large scale datasets behind current AI demonstrating how they embed societal historical and structural injustices, d) study the seemingly neutral values of ML research and put forward 67 prominent values underlying ML research, e) examine some of the insidious and worrying applications of computer vision research, and f) put forward a framework for approaching challenges, failures and problems surrounding ML systems as well as alternative ways forward.

==> chapters/04_vision/audit_card.tex <==
\begin{figure*}
\raggedright
\begin{framed}
\begin{center}{\LARGE {\bf Dataset audit card - ImageNet}}\end{center} 
\vspace{-0.15in}

\begin{minipage}{.475\textwidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Census audit statistics} 
\begin{itemize}[leftmargin=*]
\item  $83436$ images with $101070-132201$ persons (Models: DEX (\cite{rothe2018deep_dex}), {InsightFace} (\cite{insight-face}))
% \item Estimated number of human subjects: $101070-132201$
\item Mean-age (male): 33.24 (Female):25.58 ( RetinaFace \cite{deng2019retinaface}, ArcFace \cite{deng2018arcface})
\item Confirmed misogynistic images: 62. Number of classes with infants: 30
\item (${\mu _c^{(A)}}$ and ${\sigma_c^{(A)}}$: Mean and standard-deviation of the gender-estimate of images in class $c$ estimated by  algorithm $(A)$.)
\end{itemize}

% Key: $\left\{ {n/N} \right\}_{\{ train/val\}  - \{ O/W/M\} }^{(\left\{ {dex/if} \right\})}$

% (O:Overall,W:Women,M: Men)
%  $N_{train-O}^{(dex)}$=132201,$n_{train-O}^{(if)}$ =80340,$n_{val-O}^{(if)}$=3096,$N_{train-O}^{(if)}$ =97678,$N_{val-O}^{(if)}$ =3392,  $N_{train-W}^{(if)}$= 26195, $N_{train-M}^{(if)}$ 
%  =71439, $N_{val-W}^{(if)}$ =645 and  $N_{val-M}^{(if)}=  2307$. 
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.15in}
\raggedleft
\begin{minipage}{.475\textwidth}
{\bf Metrics:} 
% To begin, we denote $\phi_i$ to be the binary \textit{face-present} indicator variable\footnote{
% \[
% \begin{gathered}
%   {\phi _i} = 1\quad if\;face\;present \hfill \\
%   \quad  = 0\;otherwise \hfill \\ 
% \end{gathered} 
% \]
% } with regards to the image indexed $i$, 
% $(A)$ (in the superscripts) to be the algorithm used ($A \in \{\texttt{DEX,INSIGHTFACE}\}$), and $N_c$  to be the number of images in the class $c$. 
Class-level mean count ($\eta _c^{(A)}$), mean gender  \ \ \ \    skewness ($\xi _c^{(A)}$) and mean-age ($\alpha_c^{(A)}$): \begin{align*} 
\eta _c^{(A)} = \frac{1}{{{N_c}}}\sum\limits_{i = 1}^{{N_c}} {I[{\phi _i}]} , \alpha _c^{(A)} = \frac{1}{{{N_c}}}\sum\limits_{i = 1}^{{N_c}} {I[{\phi _i}]a_i^{(A)}} \;and\;\\
\xi _c^{(A)} = \frac{1}{{{N_c}}}{\sum\limits_{i = 1}^{{N_c}} {I[{\phi _i}]\left( {\frac{{g_i^{(A)} - \mu _c^{(A)}}}{{\sigma _c^{(A)}}}} \right)} ^3} 
\label{eq:metrics_scatter}
\end{align*} 
\ \ \  \ \ \ $
{\phi _i} = 
     \begin{cases}
       \text{1} &\text{if face present }\\
       \text{0} &\text{otherwise} \\
     \end{cases}
$
 in $i^{th}$ image.
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
  \centering
  \includegraphics[width=0.95\textwidth, height=1.95in]{plots/census/1b_dex_if_comparisons.pdf}
  \caption{Class-wise cross-categorical scatter-plots across the cardinality, age and gender scores}
  \label{fig:cag_card}
\end{figure}
\vspace{-0.35in}
\begin{figure}[H]
  \centering
  \includegraphics[width=0.9\textwidth, height=1.95in]{plots/census/2_AGN_guided.pdf}
  \caption{Statistics and locationing of the hand-labelled images}
  \label{fig:agn_card}
\end{figure}
\vspace{-0.35in}
\begin{figure}[H]
  \centering
  \includegraphics[width=0.9\textwidth, height=1.75in]{plots/census/breed_music.pdf}
  \vspace*{-2mm}
  \caption{Known \textit{human co-occurrence} based gender-bias analysis}
  \label{fig:co_occur_card}
\end{figure}
% \begin{figure}[H]
% \centering
% \captionsetup{justification=centering}
% \subfloat[Categorized violin plot demonstrating the class-wise mean gender scores across the dog-breed image groups]{
%   \includegraphics[width=0.5\textwidth]{plots/census/4a_dog_breeds.pdf}
% }
% \subfloat[Gender skewness scores across the different musical instrument image classes ]{
%   \includegraphics[width=0.5\textwidth]{plots/census/4b_music_skewness.pdf}
% }
% \caption{Known \textit{human co-occurrence} based gender-bias analysis}
% \label{fig:co_occur_gender_bias_card}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{framed}
% \vspace*{-5mm}
\caption{Dataset audit card for the ImageNet dataset}
\label{fig:audit_card}
\end{figure*}





==> chapters/08_Understanding/thick.tex <==
\chapter{Thick Data}
\label{thick}
\TODO{add a paragraph summarizing what this chapter is about}

\section{Introduction}
At the center of most scientific endeavors stands the desire to produce generalizable knowledge based on abstracted similarities, patterns, and commonalities which then allow for prediction. This relies on supposedly disentangling a complex phenomenon from its historical and contextual contingencies, stabilizing dynamic and continual processes, finalizing open and non-totalizable phenomena and bringing it down to its abstract ``essense'' or single representation. By supposedly disentangling contingencies and boiling a phenomena down to its abstract ``essense'', one can imply to get at free-standing knowledge or even truth that apply regardless of time or context. This desire for free-standing knowledge ``uncontaminated'' by particular culture, history, and context is largely inherited from the Newtonian worldview that dominates much of Western (both natural and human) science. Such worldviews stand at odds with the reality of how complex phenomena unfold but provide a way (albeit illusory) to control, manipulate, and predict complex behaviour. 

This aspiration exists in tension with gaining in-depth and contextual understanding of people and society. While most domains of enquiry that deal with people and society tread some balance between prediction and understanding, data science and machine learning stand firmly on the former. Much of current statistical and mathematical modelling operate on de-contextualization and abstraction which then allow generalizations and predictions. Predictions are often taken as probabilistic truths and yet are detached from the specific humans and societies that they are made on. With such data and modelling practices, bigger and more data is seen as a substitute for causal understanding. As we have seen in \ref{prioritizing understaning}, algorithmic injustice suffered by minoritized communities is partly rooted in the fields’ fetishization of prediction with limited understanding of people, society, histories, and structural injustices. This chapter leans on the field of cultural anthropology, specifically Geertz’s method of \textit{thick description} -- describing a phenomena with as much detail as possible with the aim of understanding (not to drive generalizations or make predictions) -- and put forward the concept of \textit{thick data} as a means to equitable ML models that primarily provides understanding of a subject of study.





%This requires a fundamental shift from a focus on striving for uniformity towards a technology that underpins 
\TODO{continue from here}





\section{Understanding vs predicting} 



\TODO{Continue from here}

deeper data \cite{brock2015deeper}

Questions regarding what the central objectives of science should be, are central concerns to the philosophy of science. For the most part, Western science aspires to get at generalizations and fundamental laws that remain constant regardless of context and time in an ``objective'' and ``view from nowhere'' manner. 

Any generalization can only be made from within a certain framing and is inherently linked to the observer, yet such an approach poses a problem for the rational worldview, for it introduces some necessary conditions, specific perspectives, and subjectivities. Treating phenomena as ahistorical and acontextual, rendering the observer invisible, is in a sense what signifies the rationalist's conception of “objective” science.

The task of finding shared similarities among differences, and repeated and recurring patterns, supposedly not only enables us to generalize, it also allows us to make predictions. However, such endeavour, as Elisabeth Roudinesco \cite{roudinesco2008philosophy} [p.xi], outlines, is shallow and devoid of critical thought: “classify, rank, calculate, measure, put a price on, normalize; this is the absolute nadir of contemporary interrogation, endlessly imposing itself in the name of a bogus modernity that undermines every form of critical intelligence grounded in the analysis of the complexity of things and persons” 

%abstracting what supposedly captures the core

%Justifiably, finding general patterns is crucial to science, at least to how science is traditionally conceived within the Western tradition. And science as traditionally conceived is interested in what remains similar in wide range of different phenomena (not what particular feature differentiates one phenomenal or person from another). 

Nonetheless, this is not claim that all attempts to find generalizable laws and make accurate predictions are deemed to fail. 

The physical sciences have been relatively successful in establishing fundamental generalizable laws, granting the power to predict astronomical moves with incredible precision, for example. The human sciences however, are far from any such universal principles that could apply to “human nature” – cognition, behaviour, morality, ethics – regardless of time, place and context. Investigation and understanding of living, sentient, cultural and historical organisms requires a radically different approach to that of inanimate objects. 


\section{The irremovable tension between the general and the particular}
\TODO{replace with Understanding social systems and cultures}

The tension between the desire to generalize and the need to gain deep understanding is a feature of most domains of enquiry that deal with the human sciences. Within cultural anthropology, these opposing positions have been highlighted by two of the field’s giants.

Cultural anthropology, according to Lévi-Strauss, at its core needs to engage in finding similar patterns across an immense range of various cultures. The task of the anthropologist, Lévi-Strauss insists, is not to account for why a culture takes a particular form, but to “understand and illustrate the principles of organisation that underlie the onward process of transformation that occurs as carriers of the culture solve problems that are either practical or purely intellectual.” Systematicity, organization, and structure preoccupied Levi-Strauss’s anthropology in his search for generalizable patterns. 

Cultural anthropology, Lévi-Strauss insists, is an endeavour in search of similarities between cultures. These similarities, he anticipates, might reveal human thought processes and uncover deep structures beneath the surface through systems of classification. The quest for overall universal patterns is more important than inscriptions of a given culture in a given context and at a given location and time, as far as Lévi-Strauss is concerned. 

Clifford Geertz, on the other hand, saw such endeavour as futile. The objective of cultural anthropology, or any field that seeks to understand humans, should more than anything else aim to understand through ‘thick description’. Cultural anthropology, Geertz argues, needs “to thickly describe with the aim of understanding”, not to make generalizations or predictions. 

Describe to what end, if not to make generalizations or discover underlying principles? For Geertz, describing a phenomenon or a culture as deeply as possible is key to understanding. And understanding in and of itself, for Geertz, is an important and sufficient objective to study cultures, phenomena, or people. Deep understanding makes successful communication, dialogue, and negotiation possible. Furthermore, understanding people's culture exposes their normalness without reducing their particularity. Deep understanding renders cultures, people and their actions and behaviours logical. It makes cultures and people that might have seemed peculiar from the outside, accessible by dissolving their opacities. 

Geertz wrote: “… I have never been impressed with claims that structural linguistics, computer engineering or some other advanced form of thought is going to enable us to understand men without knowing them.”

Geertz points out that the desire to generalize and theorize comes at the price of penetrating and gaining deep understanding of the unfamiliar. Geertz calls this conflict between the wish to theorize on the one hand, and the need to describe on the other hand, an “irremovable tension”. The further the theoretical development goes, the deeper the tension becomes. Geertz contests that theories and generalizations inevitably lack deep and contextual understanding of human thought. In his view, theoretical disquisitions stand far from the immediacies of social life and any generalizations or theory construction in the absence of deep understanding grounded in the particular is vacuous. 

Contrary to Lévi-Strauss, Geertz strongly opposed the idea that one can find simplified “typical” small towns, villages, or societies. “If anthropological interpretation is constructing a reading of what happens, then to divorce it from what happens – from what, in this time or that place, specific people say, what they do, what is done to them, from the whole vast business of the world – is to divorce it from its applications and render it vacant.” P.18 

“The major theoretical contributions not only lie in specific studies – that is true in almost any field – but they are very difficult to abstract from such studies and integrate into anything one might call ... culture theory" as such. “Theoretical formulations hover so low over the interpretations they govern that they don't make much sense or hold much interest apart from them. This is so, not because they are not general (if they are not general, they are not theoretical), but because, stated independently of their applications, they seem either commonplace or vacant.” P.25

The Russian philosopher Bakhtin held an even more radical stance in his opposition on what he calls “theoretism”. Theoretism refers to the manner in which abstract general rules are derived from concrete human actions and behaviours. Bakhtin argues such attempts to abstract general rules from particulars “loses the most essential thing about human activity, the very thing in which the soul of morality is to be found” which Bakhtin calls, the “eventness” of the event. “Eventness” is always a particular, and never exhaustively describable in terms of rules. P.7 
\TODO{tie this to how similarly, ethics is not to be inscribed into a general theory, a set of rules or...}

Bakhtin heavily criticizes the manner in which much of scientific endeavour is content with “abstract meaning”, and the fact that we are at times led to believe that that is all there is. Contrary to this, Bakhtin argues that in order to understand people, we must take into account “unrepeatable contextual meaning”. 

Theories, built on abstracted commonalities, as far as Bakhtin is concerned, are unable to tell us anything useful about individual people. Indeed, faith in generalizable rules and theories blinds us to the particular person and situation, which is where actions, behaviours and morality reside. As we theorize humans, we lose the individual act, behaviour and particular characteristics: “all attempts to overcome the dualism of cognition and life, of thought and singular concrete reality from inside theoretical cognition are absolutely hopeless…” like trying “to lift oneself up by one’s own hair” P.9 

Bakhtin believed that neither culture nor “human nature” can be made into a set of general rules and theories. He insisted that there is no substitute for an educated sensitivity to irreducibly particular people in unrepeatable particular circumstances. “The concrete act or event cannot be transcribed in theoretical terms in such a way that it will not lose the very sense of its eventness.” P. 14

\section {Minds, brains, and genomes}
\TODO{alternative heading Understanding and Human behaviour}

Alicia Juarrero has described a similar tension in the history of psychology. At its inception, psychologists concerned themselves with in-depth analysis of each individual’s history and experiences as a means of understanding their behaviour and mental habits. This is a hermeneutic approach, concerned with the interpretation of individual narratives in all their gloriously messy detail. The downside is that these interpretations can be seen as subjective, influenced also by the history of the interpreter. They necessarily include untestable inferences, given that the particulars in question could never be repeated. Aware of these limitations, a desire to be more “scientific” led psychology to search instead for “covering laws” that would explain patterns in human behaviour in general, rather than the behaviour of particular persons. 

This led to developming and embracing quantitative methods and supposedly objective metrics such as intelligence quotients or personality constructs. These are intended to isolate underlying latent variables that influence human behaviour in the abstract, summed over all individuals and all contexts. Such constructs have been shown to have some statistical power in predicting trends and patterns of behaviour as well as real-world life outcomes, when applied across large numbers of people. 

However, this does not imply any real predictive power for individuals. Any individual’s behaviour will be influenced not just by their underlying psychological predispositions, but by the very specific situations they find themselves in, and by the accumulated history of all the very specific experiences they have had in the past. It is a widespread fallacy – known as the fundamental attribution error – to ignore these particulars and the situation-dependence of behaviour, and infer instead that an individual’s behaviour at any given moment is driven primarily by their own psychological traits. 

A drive to abstract general rules is also central to much of human neuroscience, but, as in psychology, the explanatory reach and predictive power of these efforts are undermined by extensive individual variation – in this case, in the structure and function of our brains. Neuroimaging offers the power to peer into our brains to examine their structure, details of the connectivity of different regions, and even the patterns of neural activation that accompany various kinds of mental activities. These kinds of experiments have succeeded in deriving a normative map of “the human brain”, assigning functions to various areas, and helping to uncover the logic of many cognitive operations. 

The problem is this map does not apply to any actual person. The methods used to derive general patterns actively average out the rich individual differences that exist in how each of our brains are wired such as in the size and layout of different cortical areas or the connectivity of functional networks that are activated during different tasks. The details of these patterns are so idiosyncratic that they are referred to as a “neural fingerprint”. Indeed, even in an individual, the map of “functions” of cortical areas is fluid and state-dependent. 
\TODO{cite: https://www.biorxiv.org/content/10.1101/431833v2} 

Thus, attempting to predict anything definitive about individuals based on these normative patterns is futile and yet it remains a central feature of the field. This underlying heterogeneity may explain why the thousands of neuroimaging “biomarkers” that have been reported for various conditions or traits have turned out to have no diagnostic or prognostic value. 

\section{A feeling for the organism}

In all these areas of human understanding, the drive to abstract general rules runs counter to Geertz’s concept of thick description, required for deep understanding. In biology, in particular, to have one’s work described as “descriptive” became in recent times the kiss of death. Descriptive work was not just undervalued, it was often actively derided. The term was used as a pejorative, implying no real insight, no discovery of general mechanisms or principles, no point – just a lot of details. But this kind of thick description is precisely the foundation that is needed to develop a deep, almost intuitive understanding of a system – what Barbara McClintock called a “feeling for the organism”. This takes time. It requires a slow and deep immersion in the particularities of the system or phenomenon you are studying, before rushing to impose order on them by extracting laws or generalities. 

Thick description is what enabled McClintock to make the startling intellectual leap to recognise that the different colours of kernels in the corn she was studying were due to pieces of DNA that jump around in the genome. It was detailed study of individual case studies that laid the foundations for modern neurology and our conceptions of brain function. And it was decades of painstaking observations that underpinned Darwin’s discernment of the mechanism of natural selection and Ramon y Cajal’s many insights into the structural organisation of the nervous system. 

The danger now, as biology becomes more and more driven by big data, is that the feeling for the organism will be replaced by a feeling for the data – the spreadsheet, the code, the stats. Big data is seen as a substitute for deep knowledge. Why spend time (or waste time) cultivating a deep understanding of some particular system when you can abstract general patterns from “objective” data that require no expert (but often subjective) interpretation?   

Ironically, the practical consequence is that the quest for generalities washes out the particulars, undermining the goal of making predictions about individuals. Huge industries are built on the idea of applying statistical findings to individuals. This works perfectly well in insurance, where the industry is only looking for statistical outcomes. But it is a problem in areas like personalised medicine, where the outcome for individual patients becomes the key factor (at least for those patients). Organisms don’t cleave to statistical laws, except statistically. They’re messy and noisy and, above all, unique.


\section{Data science – abstraction and application}

Data science represents yet another level of abstraction away from particular bodies, histories and contexts. At the core of the field is the drive to collect or “mine” as many data points as possible and aggregate it, obscuring the rich particulars of each individual in a cloud of numbers. 

All of the above fields of enquiry and their understandings, priorities and definitions carry important implications for how we understand and treat individuals. Having said that, data science and machine learning carry the most tangible implications as they are increasingly invoked as a solution to many social problems and corporate needs. From predicting where crimes might occur or who might commit them, to monitoring employees productivity or deciding whom to hire, we seem to be happy to blindly trust patterns of data and inference made from them. For much of data science, people, behaviours, and actions entangled in contextual social, political, historical and economical milieu become a matter of abstract mathematics. Far from engaging in deep understanding, at the heart of data science is collecting, cleaning, wrangling and aggregating data with the aim of categorizing, sorting, discriminating and further predicting. 

This entails the standardisation and quantification of messy, complex and ambiguous reality, and the application of statistical algorithms to find clusters or patterns in massive amounts of data. Fluid contexts and continually changing categories are fixed as a necessary prerequisite to measurement. Multivalence, the idea that a person behaves and acts differently and moves fluidly between different categories and roles, is incompatible with this approach. Data science needs a clear definition of categories where the underlying aim is to build a model that reveals a singular truth. 

In this model of the world, with a singular truth, data science assumes a God’s eye point of view where the person behind a data point and their context, history and personal circumstances are inconsequential. This supposed “view from nowhere” in fact embodies the perspectives, motivations, interests, and biases of the data scientist themselves. 

Data science is thus at the extreme end of approaches that prioritise predictive power over understanding – indeed the black box approach of machine learning is opaque even to the operators, offering no insights as to the nature of the knowledge it has identified and applied. While the algorithms that result do indeed allow prediction across groups, they often fail when applied to individuals, precisely because the individual has been erased through the abstraction of general patterns. Moreover, in relying on statistical patterns in selected historical data, the status quo is taken as the default, with the common result that those individuals that deviate from the status quo or that don’t conform to the abstracted patterns are excluded, discriminated against, or punished.

\section{Conclusion}
The tension between abstraction and thick description is ubiquitous, and drives part of the perceived conflict between science and the humanities (C.P. Snow’s The Two Cultures).  Francis Bacon, the father of the scientific method, asserted: “Knowledge is power” – a claim that is echoed in the modern slogan: “Science – it works, bitches!”. In many areas of science, that power is defined by the ability to predict and manipulate. It is the discovery and application of general laws that lets scientists develop gene therapies for genetic disorders, create new materials an atom thick, or land a module on the surface of a comet 24 million kilometres away, traveling at 31,000 km/h. 
But when it comes to truly, irreducibly complex systems – ones that cannot be described by a small set of mathematical laws – our ability to predict from general rules is drastically more limited. This is especially true of attempts to predict the behaviour of individual human beings. The more we try to generalize, the more we leave out particulars – the unique features that differentiate a person from others, the peculiarities and idiosyncrasies that cannot be abstracted away. The more we delve into these particularities and peculiarities, the closer we come to full and deep understanding a certain person, phenomenon, or culture. These are in a sense the “why” questions that thick description allows us to tackle but that most of the dominant science shies away from. 
Our dominant scientific practices have come to overvalue abstractions, generalizations and the ability to make predictions (even when they fail to predict accurately). All of this is at the cost of devaluing describing to understand. But these approaches needn’t be seen as adversarial. Acknowledging and appreciating the complementarity of these approaches will better allow us to zoom in and out, to focus on the specific details of a phenomenon or the rich particularities of an individual, but also to explore and abstract general patterns and rules. Thick description is an essential part of science, both the foundation for generalisation and the basis for real understanding of individuals.



